Diagnostic Visualization for Deep Neural Networks Using Stochastic Gradient Langevin Dynamics

The internal states of most deep neural networks are difficult to interpret, which makes diagnosis and debugging during training challenging. Activation maximization methods are widely used, but lead to multiple optima and are hard to interpret (appear noise-like) for complex neurons. Image-based methods use maximally-activating image regions which are easier to interpret, but do not provide pixel-level insight into why the neuron responds to them. In this work we introduce an MCMC method: Langevin Dynamics Activation Maximization (LDAM), which is designed for diagnostic visualization. LDAM provides two affordances in combination: the ability to explore the set of maximally activating pre-images, and the ability to trade-off interpretability and pixel-level accuracy using a GAN-style discriminator as a regularizer. We present case studies on MNIST, CIFAR and ImageNet datasets exploring these trade-offs. Finally we show that diagnostic visualization using LDAM leads to a novel insight into the parameter averaging method for deep net training.

==> related.tex <==
\section{Related work}
\subsection{Diagnostic deep learning visualization}

There are a myriad of techniques for visualizing deep learning systems that have been presented in the last few years.  Hohman \etal \cite{hohman2018visual} provides a comprehensive survey of existing visualization techniques for understanding and diagnosing deep neural nets - however we summarize a few of the more influential here. Many recent tools focus on visualizing the neurons during training. One of the most recent tools, ActiVis \cite{kahng2018cti}, is an industry scale toolkit which allow users to perform instance and subset level inspections using clustering techniques. Their toolkit allows for analyzing and viewing clusters of neuron activations, and provides activation-level information about the images. Rauber \etal \cite{rauber2017visualizing} take a different direction by applying dimensional reduction techniques to visualize relationships between activations and between artificial neurons. Liu \etal \cite{liu2017towards} uses graph visualization to show relationship between the neurons, and visualizes their activation space. Zeng \etal \cite{zeng2017cnncomparator} uses side by side visualization to compare the activations of pairs of CNNs during training, Chung \etal \cite{chung2016re} allow users to manipulate particular neuron during training to see the training effects, and Liu \etal \cite{liu2018analyzing} analyzes the training process of deep generative models, by providing several visualizations to identify problems during training. 

While activation-level techniques can be exceptionally useful in understanding which neurons contribute to mis-classifications and understanding neural layouts (Bilal \etal \cite{bilal2018convolutional} analyzes hierarchies of similar classes to discover which neurons correspond to different levels of class hierarchy), a more general issue with many of these activation-level techniques is that they provide no way for users to understand image-level features that correspond to neuron activations. Recently, Pezzotti \etal \cite{pezzotti2018deepeyes} provides a visualization tool which allows users to view the receptive fields of neurons composed over the entire training set.  This could help users identify several diagnostic properties of a model such as stable layers, degenerated filters, undetected patterns, over-sized or unnecessary layers. However, visualizing the receptive fields using the image patches from the training set only highlights what stimulus the neuron responds to but not how it responds. In contrast, images generated by AM can give us information about the network gradient and model parameters. We will discuss the insights derived from AM in later sections as well.

%visualize regions having negative correlation with the class prediction, and can reflect the smoothness of model parameter. 

%Our proposed algorithm extends the work by Pezzotti \etal, by directly visualizing the receptive features using activation maximization instead of looking at image patches from the training dataset. There are distinct advantages to doing a direct visualization - the most important of which being that a direct filter visualization can generate images leading to high neuron activations which are not present in the training data %, leading to an ability to diagnose adversarial images, a project that is discussed further in section \textcolor{red}{TODO}. 

%Allowing users to view the receptive fields allow for the identification of a number of important %An issue with directly visualizing neuron filters using activation maximization is that these images may not be human-interpretable. This could happen for a few reasons. Perhaps the primary issue is that the activation maximization technique may achieve a local minimum which, while highly activating, is full of noise and is not human interpretable (or likely to appear in practice). To avoid the problem of visualizing what neurons respond to, Dong \etal \cite{dong2017towards} propose a method for training the filters to be directly human interpretable using adversarial examples. We borrow from this idea in section \textcolor{red}{TODO} by using a tunable discriminator to explore the boundary between adversarial images and interpretable images. 

\subsection{Activation maximization}

Central to the idea of visualizing the behavior of a neuron is the activation maximization technique. Olah \etal summarizes different activation maximization methods in \cite{olah2017feature} and describe several applications in \cite{olah2018the}. The first issue with activation-maximization is that it is underconstrained. Highly-activating images can be chosen which are visually far from the target class, as demonstrated by Szegedy \etal \cite{szegedy2013intriguing}. By starting with an image of one class, and using activation maximization, \cite{szegedy2013intriguing} showed that  adversarial examples could be created with very small perturbations in the pixel space. %Adversarial examples are images which appear to be one class, and are classified by the network as another. While sometimes adversarial examples can be helpful in diagnostics, they are extremely common, and adversarial examples that look like pure noise are neither helpful nor interpretable. 

To better constraint AM images, various regularlizers have been proposed. Mahendran \etal \cite{mahendran2016visualizing} proposed two of the most popular regularizers: total-variation (TV) regularization and jitter. Total-variation regularization penalizes images which have locally non-correlated pixels and can help with de-noising the activation-maximized image. Jitter regularization often helps to control for fine detail, and can create sharper and more vivid reconstructions. %This is particularly helpful for natural image data-sets, as the pixels in natural images are often locally correlated. A drawback of total-variation regularization is that it suffers when attempting to reconstruct intricate patterns with high image gradients. Jitter regularization falls into a larger category of transformation regularizations which ensure that the image still highly activates a neuron under transformations of the original image. Jitter regularization often helps to control for fine detail, and can create sharper and more vivid reconstructions, however using transformation regularization it can be impossible to accurately visualize neurons with transformation sensitive activation patterns (which can be useful for diagnostics in higher levels).

Besides using regularization, Nguyen \etal \cite{nguyen2016multifaceted} take the view that interpretability of the activation-maximized images is highly dependent on the initialization of the image. By using images from the training set clustered according to activation as the starting point, \cite{nguyen2016multifaceted} shows that more interpretable images can be generated. In a follow-up, \cite{nguyen2016synthesizing} uses a pre-trained generator to limit the optimization space, which then produces realistic images corresponding to higher-level activations. While the interpretability of generated images can be high, the creation of a single image is both computationally expensive and highly dependent on the generator itself, which makes it unsuitable for diagnostic purpose.  LDAM borrows the ideas presented in \cite{nguyen2016synthesizing} by replacing the generator with an adjustable adversarial discriminator. The adjustable discriminator enables LDAM to generate interpretable image samples without introducing bias in an uncontrolled manner.

Guided back-propagation \cite{springenberg2014striving} is another visualization method that also uses the gradient for the input images. It can be used to visualize the saliency map for a given input image. Smilkov \etal \cite{smilkov2017smoothgrad} improves the results from  \cite{springenberg2014striving} by adding gaussian perturbations to gradients multiple times and average the results to achieve smoother gradients. LDAM borrows the idea from \cite{smilkov2017smoothgrad} by performing sample-averaging on a series of noisy samples to improve the interpretability of the results.

%Guided BP modifies the gradient of ReLU functions by discarding the negative values of both the gradient passed from higher layers and the data passed from lower layers which means that only contributing neurons are visualized.   In addition \cite{smilkov2017smoothgrad} suggests training on data that has been perturbed with random noise to get smoother images.

%MCMC Langevin Dynamics algorithm which is able to directly sample from pixel space. Thus, the generator in LDAM is much more general, and able to clearly visualize nuances in the classifier without biasing the possible generated images in an uncontrolled manner (section \textcolor{red}{TODO}).  If the generator is not sufficiently general, then the generated images are useless for visualizing relevant input features. For example, a generator trained on one dataset could not produce useful visualizations for another dataset.

%Another issue with activation maximization is that deep neurons can be difficult to visualize due to translation invariance. In classification, a network is trying to detect members of a class, say a dog, in every part of the image. Because in a DNN every pixel can influence the target neuron through multiple hidden neurons it is possible that a pixel in one location could be highly representative of a dog is the top-left of an image, but not a dog in the bottom-right of an image, leading to a net gradient with respect to the dog neuron of 0. This issue is explored by Springenberg \etal \cite{springenberg2014striving} who propose guided backpropagation as a solution. 
\subsection{Generative Adversarial training}

Recent advances in generating realistic images have primarily been due to the introduction of adversarial training first presented by Goodfellow \etal \cite{goodfellow2014generative} in the construction of Generative Adversarial Networks (GANs). A GAN consists of two components, a generator and a discriminator. The generator $G(z) = x$ generates an image using a random input ($z$), while the discriminator $D(x)$ takes in an image $x$ and attempts to determine if $x$ is from a real dataset or was generated. By jointly training the generator and the discriminator, the generator gets better and better at ``fooling'' the discriminator, leading to more realistic images produced by the generator. In addition, the formulation for a GAN also discourages the generator from copying images that are already in the dataset. The GAN training process minimizes the Jensen-Shannon divergence between the distribution of $G(z)$ and the  distribution of training images. Zhu \etal \cite{zhu2016generative} have built an interactive toolkit which can allow users to explore such learned image manifolds in a user-controllable way. LDAM borrows a number of ideas from GANs  to improve the interpretability of the generated images, and to allow users to explore and define the interpretable image space. 

\subsection{Stochastic Gradient Langevin Dynamics}

One of the biggest problems with activation maximization techniques is that given an initialization, there is only a single maximum which can be achieved by gradient ascent. Not only is this the case, but Erhan \etal \cite{erhan2009visualizing} found that even with relatively distributed initialization, activation maximization produced only very few unique samples in practice.  This is particularly unsatisfying for visualizing images which maximize a neuron activation, because we would like to see a large number of unique images corresponding to a neuron's activation (or a cluster of neuron's activations). Thus, we would like to sample images corresponding to high activations of a neuron.  

To sample from this space LDAM borrows the optimization technique from Welling \etal \cite{welling2011bayesian}, which uses a combination of a stochastic optimization algorithm with Langevin Dynamics which injects noise into the parameter updates in such a way that the trajectory of the parameters will converge to the full posterior distribution rather than just the maximum a posteriori mode. 

A few optimizations over \cite{welling2011bayesian} have been studied. Feng \etal \cite{feng2017learning} uses Stein Variational Gradient Descent to improve the diversity of the samples drew from a posterior distribution. Neelakantan \etal  \cite{neelakantan2015adding} use gradient noise to help train deep neural nets, and Gulcehre \etal \cite{pmlr-v48-gulcehre16} propose using noisy activation function to allow the optimization procedure to explore the boundary between the degenerate (saturating) and the well-behaved parts of the activation function.


